SHAMPOO: A stochastic model for tracking dust particles under the influence of non-local disk processes

The abundances of CHNOS are crucial for the composition of planets. At the onset of planet formation, large amounts of these elements are stored in ices on dust grains in planet-forming disks. The evolution of this ice is affected by dynamical transport, collisional processes, and the formation and sublimation of ice. We aim to constrain the disk regions where these processes are fully coupled, and develop a flexible modelling approach that is able to predict the effects of these processes acting simultaneously on the CHNOS budgets of the dust in these regions. We compared timescales associated with these disk processes to constrain the disk regions where this approach is necessary, and developed the SHAMPOO code, which tracks the CHNOS abundances in the ice mantle of a single monomer dust particle, embedded in a larger aggregate and undergoing these processes simultaneously. The adsorption and photodesorption of monomer ices depend on the depth of the monomer in the aggregate. We investigated the effect of fragmentation velocity and aggregate filling factor on the amount of ice on monomers residing at r = 10 AU. The locations where disk processes are fully coupled depend on both grain size and ice species. Monomers embedded in aggregates with fragmentation velocities of 1 m/s are able to undergo adsorption and photodesorption more often compared to a fragmentation velocity of 5 m/s or 10 m/s. Aggregates with a filling factor of $10^{-3}$ are able to accumulate ice 22 times faster on average than aggregates with a filling factor of 1. As different grain sizes are coupled through collisions and the grain ice consists of multiple ice species, it is difficult to isolate the locations where disk processes are fully coupled, necessitating the development of the SHAMPOO code. The processing of ice may not be spatially limited to dust aggregate surfaces for either fragile or porous aggregates.

==> Bin/Section32_Old.tex <==
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=.9\textwidth]{Figures/32MonomerDemoDynamics.pdf}
        \caption{Evolution of the vertical position (left panel), radial position (center panel) and temperature (right panel) of a monomer released from $r=50$ AU and $z/r=0$.}
    \label{fig:32MonomerDemoDynamics}
\end{figure*}
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=.8\textwidth]{Figures/32MonomerDemoCollisions.pdf}
        \caption{Monomer collision history and resulting home aggregate size $s_a$ as a function of time. Note that the vertical position of each collision event coincides with the home aggregate size $s_a$ \textit{after} the collision has occurred.}
    \label{fig:32MonomerDemoCollisions}
\end{figure*}


As a first demonstration of the full SHAMPOO code, we consider the evolution of monomers initially at the disk midplane at $r=50$ AU in Fig. \ref{fig:32MonomerDemoDynamics}-\ref{fig:32MonomerDemoIceEvolution}. The monomer is allowed to be processed for $10^5$ yr. We assume that all home aggregates in which our monomer resides will have a constant filling factor of $\phi=0.1$. However, it should be noted that in practice the filling factor differs for each home aggregate. We therefore explore the effects of different filling factors in Sect. \ref{sec:3.3}.\\









Fig. \ref{fig:32MonomerDemoDynamics} shows the evolution of the vertical and radial position of the monomer and the monomer temperature. The monomer temperature is assumed to be equal to the local dust temperature.
In becomes clear that the monomer makes multiple vertical excursions up to $|z/r|=0.1$, while radially, the monomer tends to migrate towards the star from 50 AU down to 35 AU in 100 kyr. However, during the evolution, short radial excursions outward do occur. The net radial migration of the monomer inward results in an overall increase in monomer temperature. In addition, the three temperature peaks between $50$ kyr and $70$ kyr can be traced back to three short vertical excursions below the disk midplane (i.e. towards the disk surface).\\

\\
The combined effects of the dynamical and collisional evolution of the monomer on ice composition and elemental abundances is shown in Fig. \ref{fig:32MonomerDemoIceEvolution}. The upper left panel shows the evolution of the monomer depth $z_m$ associated with the collisional evolution depicted in Fig. \ref{fig:32MonomerDemoCollisions}. The monomer appears to have an initial period of environment exposure and a second period from approximately $50$ kyr to $70$ kyr. For most of the time the monomer is exposed, the monomer is located below the critical depth $z_m$, where we force the exposure probability to unity. It is also during these two episodes of exposure that the total monomer ice mass (upper center panel of Fig. \ref{fig:32MonomerDemoIceEvolution}) increases. This is expected since adsorption can only occur if the monomer is exposed. Within $80$ kyr, the monomer can accumulate roughly $0.25$ times its bare mass $m_m$ worth of ices. This is five times the initial total monomer ice mantle mass of $0.05 m_m$ obtained from the background model by summing over all the different initial amounts of ices obtained from Eq. \eqref{eq:initIce}. Between 90 kyr and 100 kyr, the total amount of ice on the monomer declines while the monomer is not exposed. To deduce the origin of this ice loss, we analyse the evolution of the ice mass fractions for all ice species considered (H$_2$O, NH$_3$, CO, CO$_2$, CH$_4$ and H$_2$S) in the upper right panel of Fig. \ref{fig:32MonomerDemoIceEvolution}. This panel reveals that the decrease of total ice mass between 90 kyr and 100 kyr coincides with the loss of CH$_4$ and CO ice. The loss of carbon-bearing ice can be traced back to the peak in monomer temperature between 90 kyr and 100 kyr (right panel of Fig. \ref{fig:32MonomerDemoDynamics}). The higher temperature leads to higher thermal desorption rates, and results in the total sublimation of these two ice species. Although we also consider photodesorption, the local UV flux and its effects on the photodesorption appeared to be negligible compared to thermal desorption. On one hand this is a consequence from the fact that the monomer is not exposed for most of the time. On the other hand, the background model UV flux was found to be too small throughout the entire monomer evolution to give rise to photodesorption rate which is significant when compared to the thermal desorption rate.\\
 The loss of carbon-bearing ice also affects the elemental mass fractions. The bottom left panel of Fig. \ref{fig:32MonomerDemoIceEvolution} shows that although initially the monomer ice mantle mass is dominated by oxygen and carbon, the second episode of ice formation between 50 kyr and 70 kyr results in a significant increase in the nitrogen and hydrogen ice mass fraction. This can be traced back to a significant gain in NH$_3$ ice during this episode of exposure. We also note an increase in the amount of sulfur during this episode due to the accumulation of H$_2$S. However, it should be noted that both H$_2$S and sulfur constitute only a very minor fraction of the ice mass of this monomer. Surprisingly, the loss of CO and CH$_4$ ice results in a higher S/O ratio than C/O ratio. However, due to the episode of NH$_3$ adsorption, the monomer ice mantle is chemically completely dominated by nitrogen, with the N/O ratio gradually increasing up to a value of $\sim 10$ after 100 kyr. It should be emphasized however that this does not automatically imply that all volatile solid material between $r=35-50$ AU is inclined to become dominated by nitrogen, since the above analysis pertains to the history of a single monomer. \thought{TO DO: Figure out what happens if we consider a lot of monomers... --> We do this more or less in section 4.1, although the main focus of that section is the filling factor $\phi$. I think this would transition very well into a section 3.3 where we consider the trajectories of e.g. 1000 monomers, all released from the same initial state, which allows us to make statements about the *general* processing of material originating from 50 AU. However, we may want to inform such a many-monomer-test from other work to actually use our model to help provide new insights on an actual open problem.}




{\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\textwidth]{Figures/32MonomerDemoIceEvolution1.pdf}
\end{figure*}
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=.67\textwidth]{Figures/32MonomerDemoIceEvolution2.pdf}
        \caption{Evolution of the monomer depth $z_m$ (upper left), total monomer ice mantle mass $m_\text{ice}$ (upper center), monomer ice mantle composition (upper right), the associated elemental composition (lower left) and ice molar element ratios (lower right). The line colors in the upper left panel indicate whether the monomer is exposed to the disk environment (green) or is shielded from gas phase molecules and UV photons by other monomers in the home aggregate (red).}
    \label{fig:32MonomerDemoIceEvolution}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=.8\textwidth]{Figures/33PhiSensitivity.pdf}
    \caption{Evolution of the total amount of ice (left panel) and NH$_3$ ice (right) averaged over 100 monomers for different home aggregate filling factors. Solid lines indicate the mean of the 100 monomers, whereas dashed lines indicate the standard deviation. Trajectories of individual monomers are also shown in the background.}
    \label{fig:33PhiSensitivity}
\end{figure*}}

==> Bin/Section41.tex <==






% \begin{itemize}
%     \item This model can be used to study the chemical processing of disk solids on a microscopic level. An interesting follow-up step could be to evaluate a simplified chemical network in parallel to this model. Currently we fix chemical abundances.
%     \item Processing in the inner disk: Silicate crystallization/ice crystalization. 
%     \item Statistical analysis: Since collision rates are quite low (compared to the inner disk) through most of the regions where ice is processed, we can run this code for a large population of monomers. \thought{I think this is by far the most powerful application.}. This could be applied to study questions such as
%     \begin{itemize}
%         \item How important is the non-local processing of monomers for the local dust population, and by extension, CHNOS (ice) composition.
%         \item Influence of non-local disk processing on ice structure (amorphisation/crystalization).
%         \item ...
%     \end{itemize}
% \end{itemize}






==> Bin/Section42.tex <==
We assume a constant dust size distribution as a function of position, which is just a $a_\text{pow}=3.5$ power-law distribution between some minimum size $a_\text{min}$ and maximum size $a_\text{max}$ \citep{Woitke+2016}. In reality however, $a_\text{max}$ may vary depending for which grain size relative velocities become too high. This means that the maximum grain size varies with position, and that choosing one fixed value for $v_\text{frag}$ or $a_\text{max}$ will only result the background distribution to be consistent at specific parts in the disk (see also Figure \ref{fig:23SlopeTest}). \thought{We could here also do the analysis of Section \ref{sec:2.3} at different positions to asses how bad this problem is. --> Do that once benchmarks work out.}  
